MindShift: Leveraging Large Language Models for Mental-States-Based Problematic Smartphone Use Intervention

Problematic smartphone use negatively affects physical and mental health. Despite the wide range of prior research, existing persuasive techniques are not flexible enough to provide dynamic persuasion content based on users' physical contexts and mental states. We first conducted a Wizard-of-Oz study (N=12) and an interview study (N=10) to summarize the mental states behind problematic smartphone use: boredom, stress, and inertia. This informs our design of four persuasion strategies: understanding, comforting, evoking, and scaffolding habits. We leveraged large language models (LLMs) to enable the automatic and dynamic generation of effective persuasion content. We developed MindShift, a novel LLM-powered problematic smartphone use intervention technique. MindShift takes users' in-the-moment app usage behaviors, physical contexts, mental states, goals \& habits as input, and generates personalized and dynamic persuasive content with appropriate persuasion strategies. We conducted a 5-week field experiment (N=25) to compare MindShift with its simplified version (remove mental states) and baseline techniques (fixed reminder). The results show that MindShift improves intervention acceptance rates by 4.7-22.5% and reduces smartphone usage duration by 7.4-9.8%. Moreover, users have a significant drop in smartphone addiction scale scores and a rise in self-efficacy scale scores. Our study sheds light on the potential of leveraging LLMs for context-aware persuasion in other behavior change domains.

==> data/trash/chap03-mental-states.tex <==
\section{Mental States of Habitual Smartphone Use and Intervention Strategies}

In this section, we present our approach to summarizing habitual smartphone usage mental states and designing intervention strategies. Through \textbf{a Wizard of Oz study (N=12)}, we identified that habitual smartphone usage requires intervention instead of instrumental and relaxation use. Moreover, the effectiveness of intervention is heavily influenced by users' mental states and values. Subsequently, based on findings from \textbf{semi-structured interviews (N=10) }and previous researches, we identified three mental states associated with habitual smartphone usage: \textbf{boredom, stress, and inertia}. Integrating insights from prior literature, we devised four intervention strategies: \textbf{understanding, comforting, evoking, and scaffolding habits}, and provided detailed instructions for their implementation.

\subsection{Wizard of Oz Study}

To identify specific types of smartphone use requiring intervention and develop effective persuasive content \textcolor{teal}{To identify particular smartphone usage patterns that need intervention and further develop persuasive intervention content}, we conducted a Wizard of Oz study involving 12 participants aging from 18 to 28, with an equal gender split. 


The experimental process is illustrated in Fig \ref{fig:wizard-process}. Participants were presented with a cover story in which they believed they would engage with a chatbot on WeChat, designed by us. This chatbot would monitor their smartphone usage, and upon detecting the opening of blacklisted apps, it would dispatch persuasive messages urging them to curtail usage. In reality, the WeChat account embodying the chatbot was controlled by the experimenter, entailing human-driven message generation. Upon a participant's engagement with a blacklisted app, an experimenter would be notified via email, facilitating the delivery of tailored persuasive messages based on the corresponding smartphone usage data. Subsequent to the study's conclusion, the participants were apprised of the actual nature of the experiment.

The study spanned 5 days. Each evening, researchers recorded daily interventions and conducted participant interviews, presenting them with records and inquiries. Interview topics encompassed: 1. Reasons for smartphone usage at specific times and the necessity for interventions. 2. Factors influencing acceptance of interventions. 3. Evaluation of effective persuasive content and its rationale. Upon completion of interviews and transcriptions, researchers convened daily online meetings at 22:00 to collaboratively review data and establish coding consensus.

\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]{pic/wizrd-process-min.png}
    \caption{Procedure of Wizard of Oz Study. An experimenter acts as a Chatbot behind the scene when users open any app from the restricted list.}
    \label{fig:wizard-process}
\end{figure}

\subsubsection{Habitual Smartphone Use Needs Intervention} 

We identified two distinct categories of smartphone usage, consistent with previous research: instrumental use and habitual use\cite{lukoff2018makes}. Notably, only habitual smartphone use necessitates intervention. When participants engage in instrumental phone usage and receive interventions, it can lead to dissatisfaction. For instance, participant A encountered the following intervention message: \textit{"You've already spent 1 hour and 30 minutes on WeChat today; consider putting your phone down and focusing on other aspects of life."} However, she was using WeChat for practical purposes, such as managing her affairs, rather than idly wasting time or engaging in negative behaviors. She explained her feeling, \textit{"I felt a bit resistant because the intervention message didn't align with my current context."}

We have also identified relaxation as a distinct form of instrumental smartphone use, wherein individuals purposefully employ their phones to alleviate fatigue and reward themselves following periods of intensive study or work. Intervening in such moments is deemed inappropriate. For instance, during the experiment, when the experimenter intervened with participant E, stating, \textit{"Cease scrolling through Zhihu and engage in more meaningful activities to enhance your life,"}participant E responded by saying, \textit{"This is unfounded; finding joy in scrolling through Zhihu constitutes meaning for me."} In this instance, he deliberately sought enjoyment through smartphone usage and exhibited no inclination towards intervention.

\subsubsection{Users’ Mental States and Values Matter} 

Prior researches have shown that habitual smartphone use can be linked to specific mental states, suggesting that people instinctively turn to their smartphones when experiencing certain mental states\cite{anderson2021habits,bayer2018technology}. In our study, we leveraged participants' physical context, including their app usage patterns, to infer their mental states and tailor intervention messages accordingly. Participants were also encouraged to engage in conversations with the “chatbot”, sharing their current situations. Based on daily interviews, when experimenters accurately identified and provided comfort for participants' mental states, there was an increased receptiveness to persuasive content. 

For example, in response to the message, \textit{"When you find yourself with idle time, consider engaging in meaningful activities such as reading, writing, or drawing,"} participant L noted, \textit{"It correctly identified my state of not knowing what to do and offered sensible advice"}. Additionally, in a case where participant J turned to social media due to work-related fatigue, a message suggesting, \textit{"It seems like you might need to prioritize self-care, given your mental and physical exhaustion. I suggest refraining from using your smartphones and instead trying relaxation strategies like drinking water, practicing deep breathing, or listening to music to alleviate your emotional distress and unwind,"} received a positive response, with the participant stating that she felt \textit{"very comfortable"}.

Furthermore, several participants expressed a preference for encouragement and praise, indicating that they found emotional support in such interactions.

Additionally, the researchers communicated the advantages of refraining from smartphone usage and the detriments of its prolonged use. The affirmative messages were exemplified as follows: \textit{"Elevate your gaze from WeChat; productive activities await during the evening."} Conversely, the negative messages took the form: \textit{"You're engrossed in WeChat once more, jeopardizing timely completion of your assignments."}As these messages resonated with the participants' personal values, they yielded positive evaluations. For instance, Participant M, prioritizing health, responded favorably to the message: \textit{"Your WeChat session has lasted 10 minutes; set aside your device to alleviate eye strain."} This prompted his reflection: \textit{"Undoubtedly, excessive smartphone usage detrimentally affects eyesight; I should exercise restraint."} Moreover, the researchers offered pragmatic suggestions, encouraging participants to substitute smartphone engagement with alternative actions, such as \textit{"Place your phone down and perform neck stretches."} Participants endorsed these alternatives in accordance with their values, resulting in higher ratings of the persuasive content.

\subsection{ Semi-structured Interviews }

Since the Wizard of Oz study demonstrated the susceptibility of mental states to persuasion, we sought to ascertain the prevalent mental states during habitual smartphone usage. We engaged in semi-structured interviews with 10 online-recruited participants aged 15 to 29, evenly split between genders. Participants were prompted to recollect instances of habitual smartphone use and provide insight into the underlying mental states. Professional transcription services were employed to transcribe the interviews, subsequently validated by three researchers who collaboratively identified and categorized mental states. The resulting codes coalesced into three categories: boredom, stress, and inertia. These categories demonstrated unanimity among researchers, exhibiting optimal discriminative capacity and minimal redundancy. Concurrently, existing literature corroborated the presence of these three mental states.

\subsubsection{Boredom} 

Boredom is an affective state of relatively low arousal and dissatisfaction out of an inadequately stimulating situation\cite{fisherl1993boredom,mikulas1993essence}. It fosters a habitual inclination towards automatic phone-checking, signifying that individuals tend to resort to their phones when confronted with boredom\cite{bayer2018technology}. Numerous studies underscore a substantial link between boredom and smartphone addiction, wherein the Fear of Missing Out (FOMO) acts as a mediating factor in this association\cite{bozaci2020effect,smith2015us,wolniewicz2020boredom}. This finding aligns with the outcomes derived from our semi-structured interviews, which revealed an association between habitual smartphone use and the mental state of boredom. Participants described various instances where their inclination to resort to smartphones was linked to feelings of boredom. Three distinct scenarios emerged from their narratives.

Firstly, participants noted that when the ongoing activity failed to strike a balance between their skills and the challenges, preventing the attainment of a state of flow\cite{csikzentimihalyi1975beyond}, there was the tendency to resort to smartphones. For example, participant 1 mentioned, \textit{"Memorizing vocabulary can be tedious, as it requires minimal cognitive engagement. Consequently, I find myself reaching for my phone to seek some stimulation"}. Participant 3 echoed that tasks heavy on physical activity but light on cognitive engagement were easily leading to smartphone use.

Secondly, disinterest in the current activity served as another driving factor. This disinterest could stem from a lack of intrinsic appeal, characterized by repetitive or uninteresting tasks. Participant 9 explained, \textit{"Engaging with statistics and creating tables can be immensely boring. In such instances, I tend to take breaks by scrolling through my phone or watching short videos while working"}. Furthermore, some participants reported that their engagement with tasks was driven more by obligation than personal desire, thereby failing to yield a sense of deep gratification upon completion. As participant 6 stated, \textit{"Completing assignments doesn't offer me much positive feedback; it's more about relieving from a burden rather than a feeling of accomplishment"}. Such sentiments could potentially escalate into a broader lack of enthusiasm for life, as participant 1 expressed, \textit{"I've lost all passion, the enthusiasm for learning has waned"}.

Lastly, leisure boredom, arising when individuals have idle time without any engaging activities to partake in, was also found to prompt individuals to turn to their smartphones. Participant 8 captured this situation by sharing, \textit{"When I return to my dorm and it's not yet time to sleep, I often find myself drawn to my smartphone since there's no need to study"}. Prior research has indeed highlighted a positive correlation between leisure boredom and smartphone usage\cite{kil2021leisure}.

\subsubsection{Stress} 

The second potential mental state contributing to habitual smartphone usage, as uncovered through interviews, can be conceptualized as stress. Drawing from prior literature, stress refers to maladaptive cognitive and behavioral responses when confronted with unpredictable and uncontrollable stimuli\cite{koolhaas2011stress}. A growing body of evidence suggests a certain degree of correlation between the intensity and patterns of smartphone use and individuals' perceived stress\cite{chiu2014relationship,samaha2016relationships,vahedi2018association}. This linkage could stem from smartphone usage serving as a coping strategy for individuals in dealing with stress, wherein emotional support seeking, information seeking, and self-distraction temporarily yields gratification and emotional relief\cite{duvenage2020technology}. 

Our interviews corroborate findings from previous research, as multiple participants explicitly mentioned employing smartphones due to \textit{“experiencing high levels of stress"}. Some participants attributed their smartphone use to tasks surpassing their capabilities, leading to stress from confronting uncontrollable stimuli. For instance, participant 3 remarked, \textit{"The task is too challenging, and I can't locate the bug"}, while participant 9 noted, \textit{"One day, work wasn't progressing well, I was frustrated and perplexed, so I opened my phone for a quick scroll to ease my mood"}. Other participants turned to their phones due to uncertainty regarding favorable outcomes in the future. When facing unpredictable stimuli, participant 2 commented, \textit{"I feel like I might not complete the tasks, which makes me reluctant to start, hindering the first step."} Consequently, she engaged with her phone \textit{"wearily and anxiously"}.

\subsubsection{Inertia} 

The third mental state originates from the transference of the physical concept of inertia. In physics, inertia refers to the degree to which an object resists to changing its state of motion; it maintains its motion state unchanged in the absence of external forces. Previously, several psychological studies have applied this concept. For instance, decision inertia denotes a tendency to repetitively adhere to previous choices while neglecting the consequences in new contexts, resulting in irrational suboptimal selections\cite{alos2016inertia}. Another example is emotional inertia, which refers to an individual's resistance to altering their emotional state\cite{kuppens2010emotional}. Through interviews, we have identified that one of the mental states associated with habitual mobile phone usage can also be described using the concept of inertia. In the state of inertia, individuals habitually employ their phones to evade changes in their activity state. For instance, participant 1 mentioned a habitual inclination to use his phone for a while before formally engaging in study. Similarly, participant 2, upon returning home after work, intend to transition back into a focused state for reading or other activities but struggle to shift from a relaxed state; at this point, his phone becomes the tool of procrastination. Unlike boredom or stress, in the state of inertia, individuals do not experience explicit negative emotions, yet they resist transitioning to the next activity. Consequently, we propose that it should not be hastily categorized as boredom or stress, but rather should be discussed as a distinct category.

\subsection{ Strategies Design }

While the use of mobile phones is one way individuals cope with emotional fluctuations, researches have revealed that the habitual tendency to turn to smartphones as a means of escapism is, in fact, ineffective in alleviating emotions and may even hinder recovery from jealousy and worry\cite{duvenage2020technology}. Furthermore, employing smartphones as tools for emotional regulation can lead to problematic smartphone usage, which in turn, may escalate into more severe psychological issues such as depression, thereby establishing a vicious cycle. Consequently, this study aims to intervene in habitual smartphone usage triggered by specific psychological states. The dual objectives are to reduce excessive smartphone usage and assist individuals experiencing emotional fluctuations in transitioning from avoidance coping to approach coping. This intervention seeks to fundamentally transform unhealthy emotional management habits reliant on smartphone.

According to our findings of the Wizard of Oz study and the semi-structured interviews, in order to enhance the effectiveness of persuasive content, we categorize every mental state into two dimensions: with activity and without activity. The former denotes mental states triggered by explicit sources, often linked to ongoing or upcoming user activities. For instance, activities lacking challenge and engagement, displaying high repetitiveness, might induce the state of boredom; tasks exceeding the user's capability could lead to stress; and the initiation of novel tasks could evoke a sense of inertia. Within these contexts, mobile phone usage is perceived as an avoidance coping. Thus, persuasive content within this realm should be designed to aid users in re-engaging with or initiating activities, fostering a proactive approach.

In contrast, states without activity triggers are marked by a less distinct causal origin, often intertwined with broader life circumstances. For example, a lack of enthusiasm towards life might result in a feeling of boredom, while difficulty adapting to setbacks and uncertainties could lead to stress. Additionally, becoming entrapped in idleness can result in inertia. In these scenarios, persuasive content should be tailored to recommend suitable activities that can contribute to the amelioration of the prevailing mental state.

Taking mental states as the starting point, we have devised four distinct intervention strategies, namely: Understanding, Comforting, Evoking, and Scaffolding habits.

\subsubsection{Understanding} 

A fundamental step is the comprehension of the user's mental states, as exemplified by the statement, "I understand that you find gathering materials difficult and monotonous, and you are feeling down and fatigued." This strategy emphasizes empathetic comprehension without resorting to blaming users for habitual phone checking. Past literature has suggested that seeking understanding is a coping mechanism individuals employ when faced with stimuli\cite{compas2001coping}. Furthermore, expressions of sympathy and empathy in chatbots are favored over emotionally neutral advice\cite{liu2018should}.

\subsubsection{Comforting} 

Going beyond understanding, the comforting strategy aims to provide solace to users experiencing emotional fluctuations. When in a state of boredom, past literature suggested that meaningfulness should be elevated\cite{nett2010feeling}, such as enhancing the significance of ongoing activities or helping users discover positivity and purpose in their lives. When facing stress, support should address the uncontrollable and unpredictable nature of stressors. According to past literature, strategies such as encouragement, humor, acceptance, and wishful thinking\cite{compas2001coping}, are absorbed as effective stress coping mechanisms in this study. This could involve enhancing users' self-efficacy and expectations for ongoing activities or providing gentle, humorous guidance when users lack activities, fostering an optimistic outlook for the future. In the state of inertia without explicit negative emotions, the comforting strategy is not employed.

\subsubsection{Evoking} 

Based on findings from the Wizard of Oz study, aligning with users' goals and values is a compelling persuasive technique. Thus, the evoking strategy involves gathering user goals and values (e.g., maintaining physical health, achieving academic success) and generating relevant prompts to activate stored intentions and self-norms in working memory\cite{lyngs2019self}. This strategy is suitable only for scenarios involving activities, as users lacking activities inherently lack working memory. As a result, the evoking strategy is not applicable in cases where no activities are present.

\subsubsection{ Scaffolding Habits } 

Last, we encourage users to develop scaffolding habits as an alternative to habitual smartphone use\cite{lyngs2019self,pinder2018digital}. When users instinctively resort to their phones for assistance due to specific mental states, we propose guiding them towards cultivating alternative habits that align with their desired personal development. Engaging with the phone during states of boredom and stress can be considered as a form of avoidance coping. Consequently, we suggest substituting this behavior with other habits that serve as emotional buffers. For instance, during moments of difficulty, users are advised to perform shoulder and neck stretches, and brief vocabulary recitation can be recommended during periods of boredom. In cases of inertia-driven behavior, phone usage often serves as a transitional activity or an idle pastime. To address this, we recommend engaging users in various activities that disengage them from this inertia. By collecting user preferences for desired habits beforehand and considering factors such as location and time of habitual phone usage, we can recommend suitable scaffolding habits. Users also possess the option to endorse or dismiss suggested scaffolding habits, enabling adjustments for subsequent habit recommendations. 

Strategies corresponding to different mental states as illustrated in Fig \ref{fig:strategy}.

\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]{pic/strategy1.png}
    \caption{Up: Mental states and corresponding strategies. Four strategies are labeled with different colors. Low: Specific instructions for different strategies. Strategies are shown in abbreviations (e.g. ABU means Activity-Boredom-Understanding, i.e. the strategy used in the mental state of boredom with activity).}
    \label{fig:strategy}
\end{figure}


==> table/tab_prompt_current.tex <==

\begin{table}[th]
\resizebox{\textwidth}{!}{%
\begin{tabular}{lllll}
\hline \hline
\multicolumn{5}{c}{\textbf{Current Status}} \\ \hline
\multicolumn{1}{c|}{\multirow{2}{*}{Physical Context}} &
  \multicolumn{4}{c}{Mental State} \\ \cline{2-5} 
\multicolumn{1}{l|}{} &
  \multicolumn{1}{c|}{Task-triggered frustration} &
  \multicolumn{1}{c|}{Task-triggered boredom} &
  \multicolumn{1}{c|}{Procrastination} &
  \multicolumn{1}{c}{Idleness} \\ \hline
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}It is currently "time" a.m. The \\ user has used their phone for a \\ total of "duration" minutes today \\ and last opened their phone "number" \\ minutes ago. The user completed a \\ task in the "location". \end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}The user is experiencing \\ difficulty completing their \\ task, which is causing them \\ to feel overwhelmed and open \\ their phone.\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}The user finds the task to \\ be boring, which is causing \\ them to open their phone.\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}The user is preparing to \\ start the task but wants \\ to use their phone for a \\ while before beginning.\end{tabular}} &
  \begin{tabular}[c]{@{}l@{}}The user currently has nothing \\ to do, which is causing them \\ to open their phone.\end{tabular} \\ \hline \hline
\end{tabular}%
}
\caption{Prompt Templates Designed for The Physical Contexts and The Four Mental States.}
\label{tab:prompt_current}
\end{table}
